Measurements of the branching fractions of semileptonic $D^{+}_s$ decays via $e^+e^-\to D_s^{*+}D_s^{*-}$

We measure the absolute branching fractions of semileptonic $D^+_s$ decays via the $e^+e^-\to D_s^{*+}D_s^{*-}$ process using $e^+e^-$ collision data corresponding to an integrated luminosity of $10.64~\mathrm{fb}^{-1}$ collected by the BESIII detector at center-of-mass energies between 4.237 and 4.699 GeV. The branching fractions are ${\mathcal B}(D_s^+\to \eta e^+\nu_e)=(2.35\pm0.11_{\rm stat}\pm 0.10_{\rm syst})\%,$ ${\mathcal B}(D_s^+\to \eta^\prime e^+\nu_e)=(0.82\pm0.09_{\rm stat}\pm 0.04_{\rm syst})\%,$ ${\mathcal B}(D_s^+\to \phi e^+\nu_e)=(2.21\pm0.16_{\rm stat}\pm 0.11_{\rm syst})\%,$ ${\mathcal B}(D_s^+\to f_0(980) e^+\nu_e,f_0(980)\to\pi^+\pi^-)=(0.15\pm0.02_{\rm stat}\pm 0.01_{\rm syst})\%,$ ${\mathcal B}(D_s^+\to K^0 e^+\nu_e)=(0.24\pm0.04_{\rm stat}\pm 0.01_{\rm syst})\%,$ and ${\mathcal B}(D_s^+\to K^{*0} e^+\nu_e)=(0.19\pm0.03_{\rm stat}\pm 0.01_{\rm syst})\%.$ These results are consistent with those measured via the $e^+e^-\to D_s^{*\pm}D_s^{\mp}$ process by BESIII and CLEO. The hadronic transition form factors $D^+_s\to \eta e^+\nu_e$, $D^+_s\to \eta^\prime e^+\nu_e$, and $D^+_s\to K^0 e^+\nu_e$ at four-momentum transfer squared $q^2$ = 0 are determined to be $f^{\eta}_+(0) = 0.482 \pm 0.011_{\rm stat} \pm 0.009_{\rm syst}\pm0.004_{\rm input},$ $f^{\eta^{\prime}}_+(0) = 0.562 \pm 0.031_{\rm stat} \pm 0.014_{\rm syst}\pm0.003_{\rm input},$ and $f^{K^0}_+(0) = 0.624 \pm 0.052_{\rm stat} \pm 0.013_{\rm syst}\pm0.002_{\rm input}.$

==> acknowledgement_2024-01-26.tex <==
%% Saved at => 2024-01-26
Acknowledgement
The BESIII Collaboration thanks the staff of BEPCII and the IHEP computing center for their strong support. This work is supported in part by National Key R&D Program of China under Contracts Nos. 2020YFA0406300, 2020YFA0406400, 2023YFA1606000; National Natural Science Foundation of China (NSFC) under Contracts Nos. 11635010, 11735014, 11935015, 11935016, 11935018, 12025502, 12035009, 12035013, 12061131003, 12192260, 12192261, 12192262, 12192263, 12192264, 12192265, 12221005, 12225509, 12235017, 12361141819; the Chinese Academy of Sciences (CAS) Large-Scale Scientific Facility Program; the CAS Center for Excellence in Particle Physics (CCEPP); Joint Large-Scale Scientific Facility Funds of the NSFC and CAS under Contract No. U1832207; 100 Talents Program of CAS; The Institute of Nuclear and Particle Physics (INPAC) and Shanghai Key Laboratory for Particle Physics and Cosmology; German Research Foundation DFG under Contracts Nos. 455635585, FOR5327, GRK 2149; Istituto Nazionale di Fisica Nucleare, Italy; Ministry of Development of Turkey under Contract No. DPT2006K-120470; National Research Foundation of Korea under Contract No. NRF-2022R1A2C1092335; National Science and Technology fund of Mongolia; National Science Research and Innovation Fund (NSRF) via the Program Management Unit for Human Resources & Institutional Development, Research and Innovation of Thailand under Contract No. B16F640076; Polish National Science Centre under Contract No. 2019/35/O/ST2/02907; The Swedish Research Council; U. S. Department of Energy under Contract No. DE-FG02-05ER41374
Other Fund Information
To be inserted with an additional sentence into papers that are relevant to the topic of special funding for specific topics. Authors can suggest which to Li Weiguo and/or the physics coordinator.
Example added sentence: This paper is also supported by the NSFC under Contract Nos. 10805053, 10979059, ....
National Natural Science Foundation of China (NSFC), 10805053, PWA
National Natural Science Foundation of China (NSFC), 10979059, Lund弦碎裂强子化模型及其通用强子产生器研究
National Natural Science Foundation of China (NSFC), 10775075,
National Natural Science Foundation of China (NSFC), 10979012, baryons
National Natural Science Foundation of China (NSFC), 10979038, charmonium
National Natural Science Foundation of China (NSFC), 10905034, psi(2S)->B Bbar
National Natural Science Foundation of China (NSFC), 10975093, D 介子
National Natural Science Foundation of China (NSFC), 10979033, psi(2S)->VP
National Natural Science Foundation of China (NSFC), 10979058, hc
National Natural Science Foundation of China (NSFC), 10975143, charmonium rare decays

%% ends here %%

